Cross-training with Imperfect training Schemes

Cross-training workers is one of the most efficient ways to achieve flexibility in manufacturing and service systems to increase responsiveness to demand variability. However, it is generally the case that cross-trained employees are not as productive as employees who are originally trained on a specific task. Also, the productivity of the cross-trained workers depend on when they are cross-trained. In this work, we consider a two-stage model to analyze the affect of variations in productivity levels of workers on cross-training policies. Our results indicate that the most important factor determining the problem structure is the consistency in productivity levels of workers trained at different times. As long as cross-training can be done in a consistent manner, the productivity differences between cross-trained workers and workers originally trained on the task plays a minor role. We also analyze the effect of the variabilities in demand and producivity levels. We show that if the productivity levels of workers trained at different times are consistent, the decision maker is inclined to defer the cross-training decisions as the variability of demand or productivity levels increases. However, when the productivities of workers trained at different times differ, the decision maker may prefer to invest more in cross-training earlier as variability increases.

==> figure1.latex <==
\setlength{\unitlength}{2960sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(8712,6286)(1,-6935)
\thinlines
{\color[rgb]{0,0,0}\put(2401,-6661){\vector( 0, 1){6000}}
}%
{\color[rgb]{0,0,0}\put(2401,-6661){\vector( 1, 0){6300}}
}%
{ \color[rgb]{0,0,0}\multiput(4276,-6661)(0.00000,45.00000){56}{\makebox(2.2222,15.5556){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
}%
{\color[rgb]{0,0,0}\put(5251,-6661){\line( 0, 1){2475}}
\put(5251,-4186){\line(-1, 0){2850}}
}%
{\color[rgb]{0,0,0}\put(6076,-6661){\line( 0, 1){1650}}
}%
{\color[rgb]{0,0,0}\put(2401,-3211){\line( 1, 0){1875}}
}%
{\color[rgb]{0,0,0}\put(2330,-4186){\line( 1, 0){2850}}
}%
{\color[rgb]{0,0,0}\put(4276,-3211){\line( 1,-1){975}}
}%
{\color[rgb]{0,0,0}\put(4276,-3211){\line(-1, 1){1875}}
}%
{\color[rgb]{0,0,0}\put(6076,-5011){\line( 1,-1){1650}}
}%
{\color[rgb]{0,0,0}\put(6451,-6736){\makebox(2.2222,15.5556){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
}%
{\color[rgb]{0,0,0}\put(5251,-4186){\line( 0, 1){3000}}
}%
{\color[rgb]{0,0,0}\put(5251,-4186){\line( 1, 0){2475}}
}%
{\color[rgb]{0,0,0}\put(4276,-3211){\line( 0, 1){1950}}
}%
{\color[rgb]{0,0,0}\put(6076,-5011){\line( 1, 0){1650}}
}%
{\color[rgb]{0,0,0}\multiput(2401,-5011)(45.23810,0.00000){64}{\makebox(2.2222,15.5556){\SetFigFont{5}{6}{\rmdefault}{\mddefault}{\updefault}.}}
}%
{\color[rgb]{0,0,0}\put(5251,-4186){\line( 1,-1){825}}
}%
{\color[rgb]{0,0,0}\put(4276,-3211){\line( 1, 0){3450}}
}%
\put(7051,-6886){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\alpha}+\tilde{\delta}^1_{\alpha}x^1_{\alpha}+\tilde{\delta}^2_{\alpha}(x^0_\gamma-x^1_{\alpha})$}%
}}}}
\put(3826,-6886){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\alpha}-x^1_{\gamma}$}%
}}}}
\put(4951,-6886){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\alpha}$}%
}}}}
\put(5851,-6886){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\alpha}+\tilde{\delta}^1_{\alpha}x^1_{\alpha}$}%
}}}}
\put(  101,-1411){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\gamma}+\tilde{\delta}^1_{\gamma}x^1_{\gamma}+\tilde{\delta}^2_\gamma(x^0_\alpha-x^1_\gamma)$}%
}}}}
\put(1450,-3211){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\gamma}+\tilde{\delta}^1_{\gamma}x^1_{\gamma}$}%
}}}}
\put(1601,-5011){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\gamma}-x^1_{\alpha}$}%
}}}}
\put(2056,-4186){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x^0_{\gamma}$}%
}}}}
\put(8401,-6511){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{d}_{\alpha}$}%
}}}}
\put(2101,-811){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{d}_{\gamma}$}%
}}}}
\put(3751,-5461){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_1^a$}%
}}}}
\put(6451,-6136){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_2^a$}%
}}}}
\put(7576,-5836){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_2^b$}%
}}}}
\put(6226,-4636){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_3$}%
}}}}
\put(3376,-1786){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_5^b$}%
}}}}
\put(4576,-2536){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_4^b$}%
}}}}
\put(4651,-3511){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_4^a$}%
}}}}
\put(6376,-2911){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_6^b$}%
}}}}
\put(6376,-3736){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_6^a$}%
}}}}
\put(3001,-3811){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_1^c$}%
}}}}
\put(5476,-5536){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_1^b$}%
}}}}
\put(3001,-2700){\makebox(0,0)[lb]{\smash{{\SetFigFont{9}{10.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Omega_5^a$}%
}}}}
\end{picture}%

